A Closed-Loop Perception, Decision-Making and Reasoning Mechanism for Human-Like Navigation

Reliable navigation systems have a wide range of applications in robotics and autonomous driving. Current approaches employ an open-loop process that converts sensor inputs directly into actions. However, these open-loop schemes are challenging to handle complex and dynamic real-world scenarios due to their poor generalization. Imitating human navigation, we add a reasoning process to convert actions back to internal latent states, forming a two-stage closed loop of perception, decision-making, and reasoning. Firstly, VAE-Enhanced Demonstration Learning endows the model with the understanding of basic navigation rules. Then, two dual processes in RL-Enhanced Interaction Learning generate reward feedback for each other and collectively enhance obstacle avoidance capability. The reasoning model can substantially promote generalization and robustness, and facilitate the deployment of the algorithm to real-world robots without elaborate transfers. Experiments show our method is more adaptable to novel scenarios compared with state-of-the-art approaches.

==> approach_back.tex <==
\section{Approach}
In this section, we first introduce the perception, reasoning, and decision-making components, and then provide a mathematical derivation based on the $ {\left\{o_{t},a_{t} \right\}}_{t=1:N}$ pair data collected via the optimal decision-making strategy. Finally, we describe in detail the learning process of VAE-Enhanced Demonstration learning and RL-Enhanced Interaction learning.
\subsection{Problem Formulation}
In previous approaches, the model directly maps external observations into actions. In fact, these observations also contain lots of irrelevant information and some measurement noise. So we use $o_{t}$ to denote the current observation, $a_{t}$ for current action, and $s_{t}$ for current latent state based on all observations. The truly valid features are extracted from the observation and compressed into the latent state.   

Similar to human-like navigation, perception and reasoning are two encoders based on current and historical sequences, while decision-making is a simple decoder depending on the current latent state. This process is analogous to the process in the human mind that the perception and reasoning are based on long-term memory, while decision making is an instant subconscious response. We define three models as follows:  

\textbf{Perception component}. The perception model is a sequence encoder $P$ that maps observations sequences $O_{t-n:t}$ into the latent state distribution $D_{t}^{P}$, where $O_{t-n:t}=o_{t-n} \cdots o_{t}$ denotes the sequences of observation, and latent state is sampled from this distribution, i.e. $s_{t}^{P} \sim D_{t}^{P}$. The perception model extracts useful features from the observed sequences in memory, and compresses them into the latent state, filtering out the irrelevant information.


\textbf{Decision-Making component}. The decision model is a direct mapping from latent states to actions, i.e. $a_{t}=D\left(s_{t}\right)$.

\textbf{Reasoning component}. The reasoning model $R$ is to deduce the latent state distribution $D_{t}^{R}$ based on the action sequence $A_{t-n:t}$, where $A_{t-n:t}=a_{t-n} \cdots a_{t}$ represent the sequences of actions and latent state is sampled from this distribution, i.e. $s_{t}^{R} \sim D_{t}^{R}$. The reasoning process is similar to a blind person imagining the surrounding scenes based on his own movements.

\textbf{Exploit prior data for pre-training}. 
Using DRL to directly train navigation strategies from scratch  is inefficient and expensive since DRL usually encounters a cold start problem. So we firstly pre-train the whole system with a small number of the pair data. Through pre-training, the three models have learned simple rules and knowledge.

Given some pair data$ {\left\{o_{t},a_{t} \right\}}_{t=1:N}$ sampled from optimal policy(planning algorithm) in static scene, $p(s|o)$ means perception model and $p(a|s)$ represents reasoning model. Latent state cannot be observed, inspired by \cite{li2020closed}, we calculate the likelihood of $p(a|o)$ as follows:
%
\begin{small}
\begin{equation}
p(a | o) =\sum_{s} p(s, a | o)=\sum_{s}p(a | s) p(s | o)=\sum_{s}D(\cdot)P(\cdot)
\end{equation}%
\end{small}


The algorithm attempts to maximize the log-likelihood of the observed prior data $(o_{t},a_{t})$, i.e. $\log(P(a|o))$. Assume that the decision-making module is a sample rule-based model, and ${\theta}$ denotes the parameters of the perception model.
%

\begin{equation}
\begin{aligned}
&\nabla_{\theta} \log p(a | o) =\frac{1}{p(a | o)} \nabla_{\theta} p(a | o) \\
&=\sum_{s} \frac{p(a | s) p(s | o)}{\sum_{s^{\prime}} p\left(a | s^{\prime}\right) p\left(s^{\prime} | o\right)}  \nabla_{\theta} \log p_{\theta}(s | o)
\end{aligned}%
\end{equation}%

The posterior probability  $p(s | a, o)$ can be obtained:
\begin{align}
\frac{p(a | s) p(s | o)}{\sum_{s^{\prime}} p\left(a | s^{\prime}\right) p\left(s^{\prime} | o\right)} = p(s | a, o)
\end{align}%
\begin{align}
\nabla_{\theta} \log p(a \mid o) &=\sum_{s} p(s | o, a) \nabla_{\theta} \log p_{\theta}(s | o) \label{eq2}
\end{align}  

$o$, $a$, and $s$ together constitute a Directed-Acyclic-Graph, and $o$ and $a$ together determine $s$. When $s$ is unobservable, $o$ and $a$ are conditionally independent. So $p(s|o,a) \approx p(s|o)p(s|a) \approx P(\cdot)R(\cdot)$, Equation \ref{eq2} can be formulated as: 

\begin{align}
\nabla_{\theta} \log p(a \mid o)\approx \sum_{s}P(\cdot)*R(\cdot) \log P(\cdot)
\end{align}  

Assuming $P(\cdot)$ and $R(\cdot)$ are Normal distribution($N$):
\begin{align}
\nabla_{\theta} \log p(a \mid o)\approx\sum_{s}N^{P}(s|\cdot)N^{R}(s|\cdot) \nabla_{\theta}\log N^{P}(s|\cdot)  \label{eq1}
\end{align}  

% \text { s.t. } KL\left(N^{P} \mid N^{R}\right)<\varepsilon
Based on the above derivation, apparently, we need to consider both the perception and the reasoning model. Therefore, we propose a VAE-Enhanced framework to simplify this goal.

\subsection{VAE-Enhanced Demonstration Learning}
We design a VAE-Enhanced phase to learn from pair data $ {\left\{o_{t},a_{t} \right\}}_{t=1:N}$. This process is similar to imitation learning, where the reasoning model learns the implied knowledge from the data. Inspired by the idea of VAE\cite{kingma2013auto}, we design a VAE-Enhanced demonstration learning to extract a continuous mapping for three models, avoiding overfitting these sparse data. The overview of this process is visualized in Figure \ref{fig:first_stage1}. VAE-Enhanced contains two channels : 
\begin{itemize}
\item \emph{Prediction-channel}: perception and decision-making model

\item \emph{Reconstruction-VAE-channel}: reasoning and decision-making model

\end{itemize}

\begin{figure}[t]

	\centering
	\includegraphics[scale=0.8,width = 1\linewidth]{figure/first_stage.pdf}

\caption{Overview of the VAE-Enhanced Demonstration Learning}
	\label{fig:first_stage1}
\end{figure}


Two channels share one decision-making model. More concretely, given an observation sequences $o_{t-n:t}$, perception model in \emph{Prediction-channel} encodes $o_{t-n:t}$ into latent state distribution $D^{P}_{t}$, i.e. $D^{P}_{t}=P(o_{t-n:t})$, decision-making model samples a latent state $s_{t}^{P}$ from $D^{P}_{t}$, and then predicts action output $a_t$, denoted as $a_{t}^{pred}=D(s_{t}^{P})=D(s \sim P(o_{t-n:t}))$. Symmetrically, given an action sequences, reasoning model in \emph{Reconstruction-VAE} encodes $a_{t-n:t}$ into latent state distribution $D^{R}_{t}$, i.e. $D^{R}_{t}=R(a_{t-n:t})$. Decision-making model also samples another latent state $s_{t}^{R}$ from $D^{R}_{t}$, and then reconstructs action output $a_t$, denoted as $a_{t}^{reconst}=D(s_{t}^{R})=D(s \sim R(a_{t-n:t}))$. The prediction-channel can be formalized as
\begin{align}
&\mu_{t}^{P},\sigma_{t}^{P}=\operatorname{MLP}^{P}\left(\operatorname{LSTM}^{P}\left(o_{t-n:t}\right)\right)\\ 
&s_{t}^{P} \sim N\left(\mu^{P}_{t}, \sigma^{P}_{t}\right)\\
&a_{t}^{pred}=\operatorname{MLP}^{D}\left(s_{t}^{P}\right)
\end{align}    

The procedure for \emph{Reconstruction-VAE} channel is similar. The training objective can be formulated as

\begin{align}
L_{1,t}&= (a^{reconst}_{t}-a_{t})^{2} + (a^{pred}_{t}-a_{t})^{2}\\
L_{2,t}&=\operatorname{JS}\left(N\left(\mu^{P}_{t},\sigma^{P}_{t}\right) \| N\left({\mu}^{R}_{t}, \sigma^{R}_{t}\right)\right)\\
L_{3,t}&=\sum_{\Delta \in \{P,R\}}\frac{1}{2}\left(1-\log \sigma_{t}^{\Delta}+(\mu_{t}^{\Delta})^{2}+\sigma_{t}^{\Delta}\right)
%L_{3,t}&=\frac{1}{2}\left(1-\log \sigma_{t}^{\Delta}+(\mu_{t}^{\Delta})^{2}+\sigma_{t}^{\Delta}\right), \Delta \in \{P,R\}
%L^{\theta\sim\{P,R\}}_{3} &=\frac{1}{2}\left(-\log var^{\theta}+\mu^{2}_{\theta}+var^{\theta}-1\right) \\
%
%L_{4} &=\frac{1}{2}\left(-\log var^{R}+\mu^{2}_{R}+var^{R}-1\right)
%
\end{align}

The total loss is  
$L=\sum_{t}(L_{1,t}+L_{2,t}+L_{3,t})$, where $t=1,2 \cdots N$, N is the total number of samples and JS stands for Jensen–Shannon divergence. $L_{1}$ represents the prediction loss and reconstruction loss for two channels, $L_{2}$ constrains that the latent state distribution calculated by the perception and reasoning models should be similar. $L_{3}$ is regularization constraint on two latent state distributions generated by the perception and the reasoning model, respectively.

%
%$L_{3}$ and $L_{4}$ are regularization constraints on the latent state distribution generated by the perception and the reasoning model, respectively, to make it close to the standard normal distribution.
%

%In Equation \ref{eq2}, $p(s|o,a)=p(s|a)p(s|o) \approx p(s|a)^2=p(s|o)^2$, when two latent state distributions are similar. The loss of Dual-VAE is an approximation of Equation \ref{eq1} in Section 3.1, and the optimization of Dual-VAE is more simpler. 

Intuitively, two channels achieve action prediction and reconstruction, respectively, and constrain the perception and reasoning models by JS divergence. After training, navigation knowledge and obstacle avoidance rules implied in data will be encoded into model. 



\begin{figure}[]
	\centering
	\includegraphics[width = 1\linewidth]{figure/second_stage.pdf}
\caption{The reasoning model updates itself at a fixed interval by selecting high navigation-reward actions. Meanwhile, the reasoning model generate similarity reward to evaluate each action generated by the decision-making model during the interaction.}
	\label{fig:second_stage}
\end{figure}

\subsection{RL-Enhanced Interaction Learning}
After VAE-Enhanced Demonstration learning, the model is able to master some general collision avoidance rules. However, the limited training data still confines the performance of the algorithm in highly dynamic scenarios. We introduce the RL-Enhanced Interaction learning to enhance dynamic obstacle avoidance capability through proximal policy optimization(PPO)\cite{schulman2017proximal}.

In this phase, the perception and decision-making models explore the optimal actions by interacting with the environment, while the reasoning model needs to deduce the latent state distribution based on current and historical actions. The whole process is very similar to a blind person carefully exploring the outdoor environment and he always need to imagine the surrounding scene according to his own movements.  


As shown in Figure \ref{fig:second_stage}, the trained parameters from the first phase is to initialize the three models, and a value network is added to the decision-making model for PPO update. First, the current $o_{t}$ and historical observation sequences $o_{t-n:t-1}$ are concatenated together and fed into the perception model to calculate the mean $\mu_{t}^{P}$ of the latent state distribution. Since policy module in Actor-Critic involves a sampling process, we directly treat $\mu_{t}^{P}$ as the latent state $s_{t}$ without sampling. Then decision-making model(policy module) predicts the action $a_{t}^{pred}$ based on $s_{t}$. After that, the environment executes the action $a_{t}^{pred}$ and returns \emph{navigation-reward $R^{nav}_{t}$} . Simultaneously, the reasoning model infers the most likely distribution of latent state $D_{t}^{R}$=$N(\mu_{t}^{R},\sigma^{R}_{t})$ based on the current action $a_{t}^{pred}$ and the historical real actions $a_{t-n:t-1}^{real}$. The probability of $\mu_{t}^{P}$ in $D_{t}^{R}$ is treated as a \emph{similarity-reward $R^{sim}_{t}$} for evaluating the quality of the $a_{t}$. This process can be formulated as
\begin{small}
\begin{align}
&\mu_{t}^{P} =\operatorname{MLP}^{P}\left(\operatorname{LSTM}^{P}\left([o_{t};o_{t-n:t-1}]\right)\right)\\ &a_{t}^{pred}=\operatorname{MLP}^{D}\left(\mu_{t}^{P}\right)\\
&\mu_{t}^{R}, \sigma_{t}^{R}=\operatorname{MLP}^{R}\left(\operatorname{LSTM}^{R}\left([a_{t}^{pred};a^{real}_{t-n:t-1}]\right)\right)\\ 
&O_{t+1},R_{t}^{nav} = Env(a_{t}^{pred}),  R_{t}^{sim}=\operatorname{Prob} \left(\mu^{P}_{t}\mid \mu^{R}_{t}, \sigma^{R}_{t}\right) 
\end{align}
\end{small}

\textbf{Optimization for perception and decision-making}. 
The PPO is employed to optimize the perception and decision-making model via maximizing the expected cumulative reward($R^{nav}_{t}+R^{sim}_{t}$). The loss functions of perception and decision-making model are calculated as: $L^{P, D}= \alpha*L^{policy}+\beta*L^{value}-\eta*H$, where $H, L^{policy}, L^{value}$ represent the policy entropy, policy loss, and value loss in PPO update, respectively, and $\alpha,\beta,\eta$ are hyper-parameters.

\input{table}
\textbf{Optimization for reasoning}. In order to maintain the stability of the reasoning model, we design a Discount-Reward Weighed loss(DRW-Loss for short) mechanism to optimize the reasoning model asynchronously. The reasoning model is updated every 10 PPO updates. Firstly, we collect the $ \{\mu_{t}^{P},a_{t}^{pred},R_{t}^{nav}\}$ generated by perception and decision-making model during the interaction. Then, we calculate the mean squared error between $\mu_{t}^{P}$ and $s_{t}^{R}$ as a loss to optimize the reasoning model, where $s_{t}^{R}$ is sample from $D_{t}^{R}$. However, at the beginning of training, $\mu_{t}^{P}$ and $a_{t}^{pred}$ are sub-optimal or even incorrect since the policy is not good enough. Such data should be discarded instead of being used to train the reasoning model, as it may cause the model to collapse. Therefore, we calculate the DRW-Loss to stabilize the training.  

Specifically, DRW-Loss use the \emph{navigation-reward $R^{nav}_{t}$} to calculate the discounted reward $R^{discount}_{t}$. A large discount reward means the action is more valuable. So we use the $R^{discount}_{t}$ to weight the mean squared error corresponding to the ${\{\mu_{t}^{P},a_{t}^{pred}\}}$:
\begin{align}
&R_{t}^{discount} = R^{nav}_{t} + \gamma^{1}R^{nav}_{t+1}+...+\gamma^{T-t}R^{nav}_{T}\\
&L^{R}_{1,t} = R_{t}^{discount}*\Vert \mu^{P}_{t}-s^{R}_{t} \Vert_{2}
\\
&L^{R}_{2,t}=\left(1-\log \sigma^{R}_{t}+(\mu^{R}_{t})^{2}+\sigma^{R}_{t}\right)\\
&L^{R}_{t}=\lambda*L_{1,t}^{R}+L^{R}_{2,t}
\end{align}    

where $\gamma,\lambda$ are hyper-parameters. The reasoning model assesses the action generated by the perception and decision-making models through the reward $R_{t}^{sim}$. Meanwhile, the perception and decision-making models produce more pair data $\{\mu_{t}^{P}$, $a_{t}^{P}\}$ with high navigation-reward to promote the evolution of reasoning model.


